Fast Graph Generation via Spectral Diffusion

Generating graph-structured data is a challenging problem, which requires learning the underlying distribution of graphs. Various models such as graph VAE, graph GANs, and graph diffusion models have been proposed to generate meaningful and reliable graphs, among which the diffusion models have achieved state-of-the-art performance. In this paper, we argue that running full-rank diffusion SDEs on the whole graph adjacency matrix space hinders diffusion models from learning graph topology generation, and hence significantly deteriorates the quality of generated graph data. To address this limitation, we propose an efficient yet effective Graph Spectral Diffusion Model (GSDM), which is driven by low-rank diffusion SDEs on the graph spectrum space. Our spectral diffusion model is further proven to enjoy a substantially stronger theoretical guarantee than standard diffusion models. Extensive experiments across various datasets demonstrate that, our proposed GSDM turns out to be the SOTA model, by exhibiting both significantly higher generation quality and much less computational consumption than the baselines.

==> sections/ablation_noise_schedule.tex <==
\subsection{Ablation study on diffusion schedules}\label{diffusion_schedule_ablation}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.40\textwidth]{figs/noise_schedule.pdf}
    \caption{Diffusion schedules.}
    \label{noise_schedule}
\end{figure}

In this section, we empirically verify the robustness of our proposed GSDM under various types of diffusion schedules. As shown in Figure \ref{noise_schedule}, we design six representative noise schedules with the same initial and final signal-to-noise ratio (defined in \cite{song2020score,improved_ddpm}), while  exhibiting different behaviour along the diffusion process. For both VP- and VE-SDE configurations, we train our GSDM model with six representative noise schedules and we evaluate the average performance scores. Results on Community-small, Ego-small, Grid and Enzyme datasets (Figure \ref{snr_abalation}) show that our GSDM is robust to the choice of diffusion schedules, and it is able to achieve SOTA performance without deliberate noise schedule optimization.

\begin{figure*}[]
    \centering
    \includegraphics[width=0.33\textwidth]{figs/snr_abalation_ego_small.pdf}
    \includegraphics[width=0.33\textwidth]{figs/snr_abalation_grid.pdf}
    \includegraphics[width=0.33\textwidth]{figs/snr_abalation_enzymes.pdf}
    \caption{Ablation study on the choice of noise schedules.}
    \label{snr_abalation}
\end{figure*}


\begin{figure*}[h]
\vspace{-0.2in}
\centering
\begin{minipage}{0.9\linewidth}
\centering
\begin{algorithm}[H]
    \small
    \caption{ Reverse diffusion process solver by GSDM }\label{alg:symmetric_splitting}
        \textbf{Input:} Score-based models $\bm{s}_{\theta,t}$ and $\bm{s}_{\phi,t}$, number of sampling steps $M$, step size $\delta t$, transition distributions $p_{st}(\cdot|\cdot)$ of the forward diffusion in Eq.~\eqref{eq:forward_diffusion}, Langevin MCMC step size $\alpha$, scaling coefficient $\epsilon_s$ \\
        \textbf{Output:} $\bm{X}_0$, $\bm{A}_0$
    \begin{algorithmic}[1]
        \STATE $t=T$
        \STATE Sample from the prior distribution $\bm{X}_M,\!\bm{\Lambda}_M\sim p_T, \mathbf{U}\sim \mathbf{U}_0$ 
        \FOR{$m=M-1$ \textbf{to} $0$}
            \STATE $\bm{S}_{X} \leftarrow \bm{s}_{\theta,t}(\bm{X}_{m+1},\!\bm{\Lambda}_{m+1},\mathbf{U})$; \;\;
            $\bm{S}_A \leftarrow \bm{s}_{\phi,t}(\bm{X}_{m+1},\!\bm{\Lambda}_{m+1},\mathbf{U})$ \COMMENT{score computation step}
            \STATE $\bm{X}_{m+1}\leftarrow \bm{X}_{m+1} + \frac{\alpha}{2}\bm{S}_X + \epsilon_s \sqrt{\alpha}\bm{z}_X$; \;\; $\bm{z}_X\sim\mathcal{N}\left(\bm{0},\bm{I}_{X}\right)$ \COMMENT{Correction step: $\bm{X}$}
            \STATE $\bm{\Lambda}_{m+1}\,\leftarrow \bm{\Lambda}_{m+1}\, + \frac{\alpha}{2}\bm{S}_\Lambda + \epsilon_s \sqrt{\alpha}\bm{z}_\Lambda$; \;\; $\bm{z}_\Lambda\sim\mathcal{N}\left(\bm{0},\bm{I}_{\Lambda}\right)$ \COMMENT{Correction step: $\bm{\Lambda}$}
            % \STATE $t' \leftarrow t - \delta t/2$
            \STATE $\tilde{\bm{X}}_{m}\sim p_{t,t'}(\tilde{\bm{X}}_{m}|\bm{X}_{m+1})$; \;\; $\tilde{\bm{\Lambda}}_{m}\sim p_{t,t'}(\tilde{\bm{\Lambda}}_{m}|\bm{\Lambda}_{m+1})$ \COMMENT{Prediction step: action of $e^{\frac{\delta t}{2}\fop_{F}}$}
            \STATE $\tilde{\bm{X}}_{m}\leftarrow\tilde{\bm{X}}_{m} + g^2_{1,t}\bm{S}_{X}\delta t$; \;\; $\tilde{\bm{\Lambda}}_{m}\leftarrow\tilde{\bm{\Lambda}}_{m} + g^2_{2,t}\bm{S}_{\Lambda}\delta t$ \COMMENT{Prediction step: action of $e^{\delta t\fop_{S}}\,\,$}
            \STATE $t\leftarrow t-\delta t$
            \STATE $\bm{X}_{m}\sim p_{t',t}(\bm{X}_{m}|\tilde{\bm{X}}_{m})$; \, $\bm{\Lambda}_{m}\sim p_{t',t}(\bm{\Lambda}_{m}|\tilde{\bm{\Lambda}}_{m})$ \COMMENT{Prediction step: action of $e^{\frac{\delta t}{2}\fop_{F}}$}
        \ENDFOR
        \STATE $\bm{A}_0 = \mathbf{U}\Lambda_0\mathbf{U}^\mathbf{T}$ 
        \STATE \textbf{Return:} $\bm{X}_0$, $\bm{A}_0$ 
    \end{algorithmic}
\end{algorithm}
\end{minipage}
\vspace{-0.2in}
\end{figure*}







==> sections/visualization.tex <==
% \subsection{Visualization of molecule generations}\label{molecule_visualization}

In Figure \ref{fig:molecule_visualization}, we show the generated molecules that are maximally similar to certain training molecules. We compute the molecule similarity using the Tanimoto similarity based on the Morgan fingerprints, which are implemented based on REKit \cite{landrum2016rdkit}. Higher Tanimoto scores indicate that the model is able to generate more similar molecules as the training set, which reflects the learning capability of the model. As shown in the figure, comparing to GDSS model, our proposed GSDM is able to generate molecules that have more similar distribution as the molecules in the training set. 


% The graphs from the training set are randomly selected, while the 

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figs/molecules.drawio.pdf}
    \caption{Visualization of molecule generation with maximum Tanimoto similarity of GSDM comparing to the GDSS model. The left part shows randomly selected molecules from the training set of QM9 and Zinc250k datasets. For each generated molecules, we show the Tanimoto similarity value at the bottom.}
    \label{fig:molecule_visualization}
\end{figure*}



